Doublethink: simultaneous Bayesian-frequentist model-averaged hypothesis testing

Establishing the frequentist properties of Bayesian approaches widens their appeal and offers new understanding. In hypothesis testing, Bayesian model averaging addresses the problem that conclusions are sensitive to variable selection. But Bayesian false discovery rate (FDR) guarantees are sensitive to subjective prior assumptions. Here we show that Bayesian model-averaged hypothesis testing is a closed testing procedure that controls the frequentist familywise error rate (FWER) in the strong sense. To quantify the FWER, we use the theory of regular variation and likelihood asymptotics to derive a chi-squared tail approximation for the model-averaged posterior odds. Convergence is pointwise as the sample size grows and, in a simplified setting subject to a minimum effect size assumption, uniform. The 'Doublethink' method computes simultaneous posterior odds and asymptotic p-values for model-averaged hypothesis testing. We explore Doublethink through a Mendelian randomization study and simulations, comparing to approaches like LASSO, stepwise regression, the Benjamini-Hochberg procedure, the harmonic mean p-value and e-values. We consider the limitations of the approach, including finite-sample inflation, and mitigations, like testing groups of correlated variables. We discuss the benefits of Doublethink, including post-hoc variable selection, and its wider implications for the theory and practice of hypothesis testing.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {system( "latexmk -pdf \"$_[0]\"" );}
}

==> offcuts.tex <==
\section{Introduction}

Frequently, the aim of big data analysis is to explain observed outcomes by identifying a small number of explanatory variables from a large pool of candidates. Hypothesis tests play a major role in the analysis of such data, by quantifying the evidence that certain variables influence a given outcome \citep{fisher1934statistical,neyman1933ix}. However, the evidence that one variable influences the outcome often depends on which other candidates are selected for inclusion in the model. This occurs due to correlation between variables and is pervasive in data sets with large numbers of variables. Failure to account for correlation can lead to the discovery of spurious associations that are driven by third-party variables, known as confounders \citep{vandenbroucke2002history}. Such model sensitivity is especially important when the aim is to understand underlying processes, and not merely to predict an outcome. Hypothesis testing therefore needs to account for uncertainty in model selection in terms of the inclusion or exclusion of other variables.

Bayesian model averaging (BMA) offers a systematic approach to hypothesis testing that accounts for uncertainty in model selection and can be applied to big data \citep{raftery1995bayesian}. In BMA, the relative fit of the correlated variables determines their posterior odds of an effect on the outcome, versus no effect. However, this approach is currently under-utilized. In epidemiology, for example, results are often presented for a limited number of variables that have been shortlisted through a narrowly posed question or using procedures that are not always clearly stated. Automated approaches to model selection are also used, for example by scanning for univariate associations, stepwise regression, machine learning, or statistical optimization \citep{miller2002subset,porwal2022comparing}; however, none of these methods carry forward model uncertainty, as required by hypothesis testing. This makes them particularly problematic for the analysis of large-scale data.

The disinclination towards Bayesian approaches is attributable to several issues \citep{gelman2008objections}. Often, Bayesian methods are more computationally intensive than classical methods, but the major issue is the need to specify prior distributions for model parameters and their impact on conclusions. For parameter estimation, Bernstein-von Mises theorem \citep{borwanker1971bernstein} states that Bayesian and frequentist estimates and confidence regions converge for large sample sizes under certain assumptions \citep{gelman2013philosophy}. For hypothesis testing, however, the prior exerts a direct effect on the Bayesian posterior odds of an alternative hypothesis versus a null hypothesis, regardless of sample size: in certain scenarios, simply doubling the prior odds can double the posterior odds. For this reason, some analysts interpret the ratio of posterior to prior odds (the Bayes factor), but that quantity is strongly influenced by the prior distribution of the parameters \citep{gelman2013philosophy}. Partly, this is an issue of scale: the prior odds contribute a constant term to the log posterior odds that is overwhelmed by other terms in large samples -- indeed Bayesian hypothesis testing is consistent \citep{doob1949application,kass1995reference, ohagan1995fractional}. Irrespective of sample size, however, priors influence conclusions in the area of test space that is of principal concern. Ultimately, therefore, prior choices can lead different researchers to different conclusions from the same data \citep{gelman2013philosophy}.

Frequentist methods, by contrast, are not influenced by user choice in the same way. Instead, discussions on the appropriate application of frequentist hypothesis tests to ever-increasingly large and complex data centre around other topics. One is the correct choice of false-positive rate used to determine the significance threshold. Typically this is fixed at some predetermined level, such as $\alpha = 0.05$ \citep{stigler2008fisher}, and is therefore independent of sample size. Accordingly, and as highlighted by the Jeffreys–Lindley’s paradox, the test will reject a `true' null hypothesis with a non-negligible probability, $\alpha$, \citep{jeffreys1939theory, lindley1957statistical}, even for an arbitrarily large data set. For this reason, it has been argued \citep{lindley1957statistical, naaman2016almost} that test stringency should instead increase with sample size, as occurs naturally with Bayesian test procedures. 
Overall, therefore there exists a need to critically evaluate how test criteria are devised in the the context of big data. A second topic is a need to avoid practices known as data dredging or 'p-hacking', where the number of tests being carried out is larger than reported/accounted for. This concern is particularly relevant to the search for groups of significant variables amongst a large number of candidate variables, where the total number of possible tests that can be carried out is often prohibitively large.

In this paper, we address these issues by combining the benefits of Bayesian model averaging with classical hypothesis testing to tackle the problem of identifying both individual variables and groups of variables, associated with an outcome in a regression setting. Building upon theory on the use of Bayes Factors as test statistics \citep{johnson2005bayes, johnson2008properties, hu2009bayesian} our approach relies on a large sample assumption and the construction of a specific prior density on the regression parameters. With these assumptions as a foundation, we show how the theory of regular variation  \citep{karamata1933mode, mikosch1999regular} can be used to extend the idea of interconverting Bayesian posterior odds and frequentist p-values \citep{good1992bayes,zhou2018null,held2018p} to the model-averaged setting. We highlight that this enables us to pursue model-averaged hypothesis testing while simultaneously controlling the Bayesian false discovery rate (FDR) and the frequentist family-wise error rate (FWER) in the strong sense. This result is significant as it allows for different variable groupings to be explored for signals, post hoc, without resorting to 'p-hacking'. The theory also elucidates how Bayesian and frequentist test criteria relate, informing the choice of test criteria in a big data setting.

The hypothesis tests that we formulated are embedded in a new analytic approach that aims to produce simultaneous Bayesian and classical inference, in which effect size point estimates and confidence/credibility intervals converge for large sample sizes. Because the approach was designed to produce convergence between the two statistical philosophies, it is named Doublethink in recognition of Orwell's term for the ability to simultaneously and earnestly hold contradictory beliefs \citep{orwell1949nineteen}. Our framework yields a highly capable model-averaging approach that can be applied to the systematic evaluation of direct risk factors in biobank-scale resources, as we have demonstrated in a complimentary paper (reference Arning).

To explore the theoretical properties of Doublethink, here we apply it to a well-known dataset ???. We show...? ? Using this example, we discuss the limitations of our approach and its potential implications for the practice and philosophy of hypothesis testing.



\section{Discussion}



%For Discussion: In summary, therefore, we show that it is possible to pursue model-averaged hypothesis testing, while simultaneously controlling the Bayesian false discovery rate (FDR) and the frequentist familywise error rate (FWER) in the strong sense. An equivalent interpretation of these results is that the model-averaged deviance ($2 \log {R_{\mathcal{A}_{\V}:\mathcal{O}_{\V}}}$) follows a chi-squared distribution with one degree of freedom, when large. This means that Doublethink p-values cannot be arbitrarily rescaled by the prior parameters, $\mu$ and $h$, because (i) the null distribution of the model-averaged deviance does not depend on them, and (ii) the realized value depends on them only through weights. Therefore $\mu$ and $h$ influence the power of the test, but not its theoretical distribution under the null hypothesis. This makes model-averaged hypothesis testing a viable frequentist procedure by facilitating a prior-agnostic approach to quantifying Bayesian significance thresholds in terms of the FWER, for large samples.


Bayesian model averaging is an approach especially suited to accounting for model uncertainty when investigating which variables from a large number of candidate variables directly affect an outcome. Here we showed that appropriate construction of the prior allows simultaneous control of the Bayesian FDR and the frequentist FWER. Doublethink makes use of these theoretical properties and facilitates joint Bayesian/frequentist model-averaging in big data settings that justify the exploitation of computationally efficient asymptotic approximations. It interconverts model-averaged Bayesian posterior probabilities and p-values, which unlocks transparent, systematic, big-data approaches to risk factor discovery through hypothesis testing. This has the potential to assist areas of research, such as epidemiology where classical statistics predominate, by reducing the need for hard-to-scrutinize preliminary model selection and narrowly defined candidate risk factor-based approaches. Furthermore, it fills a niche that is fundamentally different from what can be achieved through machine-learning models, which seek to predict outcomes rather than test hypotheses.

Several assumptions underpin the Doublethink tests. These are: (i) a large sample size, which implies that a Normal approximation to the likelihood is reasonable; (ii) that the response data can be regarded as a set of independent realizations from multivariate random variables satisfying a list of technical conditions that imply that maximum likelihood estimators are locally unique, consistent and asymptotically Normal \citep{cox1974theoretical}; (iii) that hypothesis tests are derived based a contradictory assumption and (iv) a particular family of priors parameterized by $\mu$ and $h$.

We acknowledge that these assumptions may restrict the applicability of Doublethink.  In particular, we highlight that the prior covariance on the regression coefficients, based on Fisher information, is hard to justify except through its convenience for pursuing joint Bayesian/frequentist inference. This motivating aim is only achieved theoretically as the sample size becomes arbitrarily large. Strictly speaking, therefore, that aim is not truly met, meaning the theoretical properties of the p-value may not hold precisely, leading to inflation or deflation, particularly when the p-value is not small, and reducing robustness to poor choices of $h$ and particularly $\mu$. It is also important to highlight that the theory used to derive an expression for the posterior odds in terms of the maximized likelihood ratio is based upon a technical contradiction. The hyperparameter $h$ is initially assumed to scale with the sample size, $n$, in line with a 'local alternatives' assumption. Later, however, $h$ is assumed to be constant with respect to $n$, which affords simplifications in deriving a p-value for the model-averaged posterior odds \citep{johnson2005bayes, johnson2008properties} and ensures consistency of the tests.

Beyond its practical utility, Doublethink has wider implications for bridging the gap between Bayesian and classical philosophies to scientific inference. First, Lemma 1 showed that the Bayesian approach to testing a collection of null hypotheses $\beta_j=0,\,j\in \V$, in which the null hypothesis is rejected when the posterior odds exceed a fixed threshold, $\tau$, is a closed testing procedure \citep{marcus1976closed}, which therefore controls the frequentist FWER in the strong sense at or below some level $\alpha$. This result is general and does not depend on the Doublethink model. Importantly, it disproves the idea that the FWER is a fundamentally non-Bayesian quantity, inherently more stringent than the FDR, which the Bayesian approach controls at or below level $1/(1+\tau)$.

Second, Theorem 2 gave an analytic expression for $\alpha$, the level at or below which the FWER is controlled in the strong sense, asymptotically under the Doublethink model. From there, we could interconvert model-averaged posterior odds and adjusted p-values, and equivalently, we could interconvert FWER and FDR thresholds. This affords insights by allowing frequentist multiple testing thresholds to be understood in terms of Bayesian prior assumptions. According to Theorem 2, $\alpha$ is asymptotically proportional to $\nu\, \mu\, (h/n)^{1/2}\,\tau^{-1}$. That is, asymptotically proportional to (i) the number of variables, $\nu$, which underlies Bonferroni correction; (ii) the prior odds, $\mu$, of the alternative hypothesis versus the null; and (iii) the square root of the prior precision $h$, higher values of which make the alternative hypothesis more similar to the null. Furthermore, it is inversely proportional to (i) the Bayesian threshold, $\tau$; and (ii) the square root of the sample size, $n$. The relationship $\alpha=\alpha_0\, \nu\, \mu\, (h/n)^{1/2}$, for some constant $\alpha_0$, offers a resolution to the classical paradox about multiple testing \citep{grafen2002modern}: should  $\alpha_0$ be varied to correct for the number of tests in the analysis, in the whole paper, in the scientists' career or in the whole scientific literature? The Bayesian response is to fix $\alpha_0$ not $\alpha$, that is to fix the FDR and allow the FWER to vary depending according to $\nu$, $\mu$, $h$, and $n$.

Third, Theorem 2 thus revisits the Jeffreys-Lindley paradox \citep{wagenmakers2023history} by emphasizing a principal difference between Bayesian and frequentist hypothesis tests, not in philosophical issues like the treatment of parameters as fixed or random, but in the practical choice of significance threshold. The common practice of fixing the FWER irrespective of sample size, $n$, e.g. at 0.05 or 0.005 \citep{benjaminwagenmakers}, leads to tests that are inconsistent under the null because there is a tangible probability, $\alpha$, of wrongly rejecting the null hypothesis even for arbitrarily big data \citep{ohagan1995fractional}. This is solved by varying $\alpha$ with $n^{-1/2}$, a starting point from which one could calculate either the FWER or the FDR.

The FDR considered here is related to, but distinct from, some FDR concepts common in the literature. First, we control the Bayesian FDR, rather than a frequentist FDR, controlled by procedures like Benjamini and Hochberg’s \citep{benjamini1995controlling} or Storey’s \citep{storey2003positive}. Second, we control the local FDR, meaning we only call an individual variable significant when its posterior inclusion probability exceeds the FDR threshold, $\tau/(1+\tau)$. Typically, frequentist FDR procedures call the largest $k$ individual variables significant such that the mean FDR is controlled. This is more powerful, but it can allow a variable with low posterior probability to be called individually significant, meaning we would reject the null hypothesis that it has no direct effect; we consider this to be a mistake. Instead, we test groups of variables; not just the group containing the $k$ most significant individual variables, but arbitrary groups. When a group of variables is called significant, we reject the null hypothesis that all their direct effects are zero, without necessarily pinpointing which variables have a non-zero direct effect: this is an important difference in interpretation. In other words, the alternative hypothesis is not that all variables in the group have a non-zero direct effect, but that at least one of them has a non-zero direct effect \citep{goeman2011multiple}.

Further research is needed to determine the generalizability of some of our theoretical findings beyond the Doublethink model. The form of Theorem 2 depends on the model choice prior, in which $\mu$ is fixed. The impact of co-estimating $\mu$ requires attention. The prior on the coefficients also matters. On one hand, Doublethink may be general in that log Bayes factors for nested hypothesis tests converge asymptotically to the Schwarz criterion \citep{kass1995reference, ohagan1995fractional}, which Doublethink recapitulates when the sample size is large. On the other hand, the derivation of Theorem 2 relies heavily on the theory of regular variation \citep{karamata1933mode, mikosch1999regular}. In Doublethink, the posterior odds are regularly varying random variables, but slowly varying posterior odds arise in non-nested settings \citep{held2019bayesian, wilson2019reply}. The interconversion of p-values and posterior odds -- or equivalently FWER and FDR -- could then behave quite differently.

Doublethink is closely related to recent developments in combined hypothesis tests that exploit heavy-tailed distributions such as the Cauchy combination test \citep{liu2020cauchy} and the harmonic mean p-value (HMP; \citet{wilson2020generalized}). The HMP provides a model-averaging approach, starting with p-values, whereas Doublethink pursues joint Bayesian/frequentist model-averaging, beginning with nested maximized likelihood ratios. These are closely related, but a theoretical advance over the HMP is the ability of Doublethink to average over uncertainty in the null hypothesis, as well as the alternative hypothesis. An interesting result from Doublethink is that under the null hypothesis, the model-averaged deviance asymptotically follows a chi-squared distribution with one degree of freedom. This mirroring of the null distribution of the classical likelihood ratio test statistic emerges from the self-similarity \citep{mandelbrot1968fractional, taqqu1978representation} or ‘fractal’ property of sums of heavy-tailed random variables. Moreover, the model-averaged deviance could be interpreted instead of the posterior odds or Bayes factor, which are strongly influenced by the prior \citep{gelman2013philosophy}.

Doublethink, like the HMP, enables us to reconsider established positions concerning the philosophy and practice of hypothesis testing. In particular, the multilevel nature of these tests, in which all possible combinations of hypotheses are simultaneously controlled via pre-determined thresholds, like \citet{goeman2011multiple}, supports refinements to concepts like fishing for significance, data dredging, and p-hacking \citep{andrade2021harking}. For a fixed set of predetermined null hypotheses, Doublethink allows us to search in arbitrary ways for significant groups of variables, without impacting the FDR and, at least asymptotically, the FWER in the strong sense. Since exhaustive searches are not generally practicable, the methods by which signals are sought through grouping variables become important. In an associated application paper we showed that the groupings had a strong impact on the relative prominence of signals in identifying risk factors for Covid-19 deaths, highlighting that more work is required to evaluate different algorithms used to identify groups. From these insights and through new avenues of research, this work has the potential to help advance scientific discovery and bridge the divide between Bayesian and classical hypothesis testing.


Instead, it is an attempt to understand why, and under what circumstances, $p$-values offer sensible measures of the evidence against a null hypothesis, despite their well-advertised flaws (refs).
A central Bayesian criticism of $p$-values is their general violation of the likelihood principal, meaning that inference is based on the probability of unobserved data `as or more extreme than' the observed data.
Johnson's (refs) interconversion of LRT-based Bayes factors to $p$-values clearly preserves the evidential value of the LRT established by the Neyman-Pearson lemma.
Yet combining $p$-values ostensibly breaks this one-to-one relationship, and seems to irrevocably violate the likelihood principle.
The insight from Karamata's theory of regular variation is that combination tests based on sums of heavy-tailed random variables produce test statistics that are stochastically dominated by the maximum of those variables.
This offers a reprieve for $p$-values calculated from such tests, which include sums of heavy-tailed posterior odds, as in Doublethink, because the null distributions of their test statistics are fractal, or self-repeating.
Another serious objection to $p$-values is the focus on their performance under the null, without reference to statistical power.
Lehmann argued that even Fisher acknowledged the importance of power (e.g.\ in experimental design) but rejected the Neyman-Pearson idea you could quantify it, the relevant parameters being unknown by definition.
By combining the benefits of Bayesian and frequentist hypothesis testing, assumptions about power are incorporated directly through the prior.
In this sense, the Bayesian approach performs optimally when the prior is well-specified, but its properties under the null hypothesis can be quantified - in principal - even when the prior is wrong.
From these insights and through new avenues of research, we hope this work will help advance scientific discovery and bridge the divide between Bayesian and classical hypothesis testing.


\section{TO DO}

    \item In the Combined performance simulations, for methods other than Doublethink, how are pairwise and truenull p-values/statistics computed?
    \item In real data analysis, combining the p-values reveals no significant results.
    \item To what extent do the simulation results presented so far refer to Theorem 2 + CTP as well as Theorem 3?
    \item Combined performance simulations: investigate BFWER$_{0.5}$ and BFWER$_1$.
    \item Do standard marginal-based combination tests benefit in terms of FWER by being under-powered? Does this allow them to perform marginal tests without worrying about inflation of the FWER? Because marginally, the tests are \emph{deflated}, not inflated?
    \item Theorem 2 vs 3: test of the intersection of true nulls is pertinent to Th 3. But could also just use Th 2 with a different method of combining tests: e.g. Bonferroni, Simes, Hommel, hmp. This is less powerful - and maybe less inflated? How does the real data analysis look different?
    \item Combined performance simulations: Need to evaluate power to reject the intersection of true nulls too. This is where Th 3 should win out? Dur - cannot define power because they are always truly null. What should this be instead? Power to reject any/all of the complement of the true nulls? If I correctly reject any elementary hypothesis, I must correctly reject that the set of true alternatives are all nulls. To correctly reject *all* true alternatives I must reject all their elementary hypotheses - this is hard. So complement of the type I error of rejecting the intersection of true null hypotheses is the type II error of failing to reject the intersection of true alternative hypotheses (i.e. failing to reject that any of them are non-null). -- Need to define 'truealts' in the combined performance simulations.

    \item Worry about whether sup is over omega or Theta in various FPRs. Same thing: open vs closed sets.



==> what_left_to_do.tex <==
\begin{comment}

\begin{itemize}
\item Migrate to the journal-specific template?

\item Activate Zenodo doi 10.5281/zenodo.15360270

\item Write readme for source code at https://github.com/danny-wilson/dblthk_amd_sims

\item Mention possible editors and reviewers in the cover letter

\end{itemize}

\end{comment}
